On the Unreasonable Effectiveness of Feature propagation in Learning on Graphs with Missing Node Features

While Graph Neural Networks (GNNs) have recently become the de facto standard for modeling relational data, they impose a strong assumption on the availability of the node or edge features of the graph. In many real-world applications, however, features are only partially available; for example, in social networks, age and gender are available only for a small subset of users. We present a general approach for handling missing features in graph machine learning applications that is based on minimization of the Dirichlet energy and leads to a diffusion-type differential equation on the graph. The discretization of this equation produces a simple, fast and scalable algorithm which we call Feature Propagation. We experimentally show that the proposed approach outperforms previous methods on seven common node-classification benchmarks and can withstand surprisingly high rates of missing features: on average we observe only around 4% relative accuracy drop when 99% of the features are missing. Moreover, it takes only 10 seconds to run on a graph with $\sim$2.5M nodes and $\sim$123M edges on a single GPU.

==> math_commands.tex <==
% %%%%% NEW MATH DEFINITIONS %%%%%

% \usepackage{amsmath,amsfonts,bm}

% % Mark sections of captions for referring to divisions of figures
% \newcommand{\figleft}{{\em (Left)}}
% \newcommand{\figcenter}{{\em (Center)}}
% \newcommand{\figright}{{\em (Right)}}
% \newcommand{\figtop}{{\em (Top)}}
% \newcommand{\figbottom}{{\em (Bottom)}}
% \newcommand{\captiona}{{\em (a)}}
% \newcommand{\captionb}{{\em (b)}}
% \newcommand{\captionc}{{\em (c)}}
% \newcommand{\captiond}{{\em (d)}}

% % Highlight a newly defined term
% \newcommand{\newterm}[1]{{\bf #1}}


% % Figure reference, lower-case.
% \def\figref#1{figure~\ref{#1}}
% % Figure reference, capital. For start of sentence
% \def\Figref#1{Figure~\ref{#1}}
% \def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
% \def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% % Section reference, lower-case.
% \def\secref#1{section~\ref{#1}}
% % Section reference, capital.
% \def\Secref#1{Section~\ref{#1}}
% % Reference to two sections.
% \def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% % Reference to three sections.
% \def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% % Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% % Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% % A raw reference to an equation---avoid using if possible
% \def\plaineqref#1{\ref{#1}}
% % Reference to a chapter, lower-case.
% \def\chapref#1{chapter~\ref{#1}}
% % Reference to an equation, upper case.
% \def\Chapref#1{Chapter~\ref{#1}}
% % Reference to a range of chapters
% \def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% % Reference to an algorithm, lower-case.
% \def\algref#1{algorithm~\ref{#1}}
% % Reference to an algorithm, upper case.
% \def\Algref#1{Algorithm~\ref{#1}}
% \def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
% \def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% % Reference to a part, lower case
% \def\partref#1{part~\ref{#1}}
% % Reference to a part, upper case
% \def\Partref#1{Part~\ref{#1}}
% \def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

% \def\ceil#1{\lceil #1 \rceil}
% \def\floor#1{\lfloor #1 \rfloor}
% \def\1{\bm{1}}
% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

% \def\eps{{\epsilon}}


% % Random variables
% \def\reta{{\textnormal{$\eta$}}}
% \def\ra{{\textnormal{a}}}
% \def\rb{{\textnormal{b}}}
% \def\rc{{\textnormal{c}}}
% \def\rd{{\textnormal{d}}}
% \def\re{{\textnormal{e}}}
% \def\rf{{\textnormal{f}}}
% \def\rg{{\textnormal{g}}}
% \def\rh{{\textnormal{h}}}
% \def\ri{{\textnormal{i}}}
% \def\rj{{\textnormal{j}}}
% \def\rk{{\textnormal{k}}}
% \def\rl{{\textnormal{l}}}
% % rm is already a command, just don't name any random variables m
% \def\rn{{\textnormal{n}}}
% \def\ro{{\textnormal{o}}}
% \def\rp{{\textnormal{p}}}
% \def\rq{{\textnormal{q}}}
% \def\rr{{\textnormal{r}}}
% \def\rs{{\textnormal{s}}}
% \def\rt{{\textnormal{t}}}
% \def\ru{{\textnormal{u}}}
% \def\rv{{\textnormal{v}}}
% \def\rw{{\textnormal{w}}}
% \def\rx{{\textnormal{x}}}
% \def\ry{{\textnormal{y}}}
% \def\rz{{\textnormal{z}}}

% % Random vectors
% \def\rvepsilon{{\mathbf{\epsilon}}}
% \def\rvtheta{{\mathbf{\theta}}}
% \def\rva{{\mathbf{a}}}
% \def\rvb{{\mathbf{b}}}
% \def\rvc{{\mathbf{c}}}
% \def\rvd{{\mathbf{d}}}
% \def\rve{{\mathbf{e}}}
% \def\rvf{{\mathbf{f}}}
% \def\rvg{{\mathbf{g}}}
% \def\rvh{{\mathbf{h}}}
% \def\rvu{{\mathbf{i}}}
% \def\rvj{{\mathbf{j}}}
% \def\rvk{{\mathbf{k}}}
% \def\rvl{{\mathbf{l}}}
% \def\rvm{{\mathbf{m}}}
% \def\rvn{{\mathbf{n}}}
% \def\rvo{{\mathbf{o}}}
% \def\rvp{{\mathbf{p}}}
% \def\rvq{{\mathbf{q}}}
% \def\rvr{{\mathbf{r}}}
% \def\rvs{{\mathbf{s}}}
% \def\rvt{{\mathbf{t}}}
% \def\rvu{{\mathbf{u}}}
% \def\rvv{{\mathbf{v}}}
% \def\rvw{{\mathbf{w}}}
% \def\rvx{{\mathbf{x}}}
% \def\rvy{{\mathbf{y}}}
% \def\rvz{{\mathbf{z}}}

% % Elements of random vectors
% \def\erva{{\textnormal{a}}}
% \def\ervb{{\textnormal{b}}}
% \def\ervc{{\textnormal{c}}}
% \def\ervd{{\textnormal{d}}}
% \def\erve{{\textnormal{e}}}
% \def\ervf{{\textnormal{f}}}
% \def\ervg{{\textnormal{g}}}
% \def\ervh{{\textnormal{h}}}
% \def\ervi{{\textnormal{i}}}
% \def\ervj{{\textnormal{j}}}
% \def\ervk{{\textnormal{k}}}
% \def\ervl{{\textnormal{l}}}
% \def\ervm{{\textnormal{m}}}
% \def\ervn{{\textnormal{n}}}
% \def\ervo{{\textnormal{o}}}
% \def\ervp{{\textnormal{p}}}
% \def\ervq{{\textnormal{q}}}
% \def\ervr{{\textnormal{r}}}
% \def\ervs{{\textnormal{s}}}
% \def\ervt{{\textnormal{t}}}
% \def\ervu{{\textnormal{u}}}
% \def\ervv{{\textnormal{v}}}
% \def\ervw{{\textnormal{w}}}
% \def\ervx{{\textnormal{x}}}
% \def\ervy{{\textnormal{y}}}
% \def\ervz{{\textnormal{z}}}

% % Random matrices
% \def\rmA{{\mathbf{A}}}
% \def\rmB{{\mathbf{B}}}
% \def\rmC{{\mathbf{C}}}
% \def\rmD{{\mathbf{D}}}
% \def\rmE{{\mathbf{E}}}
% \def\rmF{{\mathbf{F}}}
% \def\rmG{{\mathbf{G}}}
% \def\rmH{{\mathbf{H}}}
% \def\rmI{{\mathbf{I}}}
% \def\rmJ{{\mathbf{J}}}
% \def\rmK{{\mathbf{K}}}
% \def\rmL{{\mathbf{L}}}
% \def\rmM{{\mathbf{M}}}
% \def\rmN{{\mathbf{N}}}
% \def\rmO{{\mathbf{O}}}
% \def\rmP{{\mathbf{P}}}
% \def\rmQ{{\mathbf{Q}}}
% \def\rmR{{\mathbf{R}}}
% \def\rmS{{\mathbf{S}}}
% \def\rmT{{\mathbf{T}}}
% \def\rmU{{\mathbf{U}}}
% \def\rmV{{\mathbf{V}}}
% \def\rmW{{\mathbf{W}}}
% \def\rmX{{\mathbf{X}}}
% \def\rmY{{\mathbf{Y}}}
% \def\rmZ{{\mathbf{Z}}}

% % Elements of random matrices
% \def\ermA{{\textnormal{A}}}
% \def\ermB{{\textnormal{B}}}
% \def\ermC{{\textnormal{C}}}
% \def\ermD{{\textnormal{D}}}
% \def\ermE{{\textnormal{E}}}
% \def\ermF{{\textnormal{F}}}
% \def\ermG{{\textnormal{G}}}
% \def\ermH{{\textnormal{H}}}
% \def\ermI{{\textnormal{I}}}
% \def\ermJ{{\textnormal{J}}}
% \def\ermK{{\textnormal{K}}}
% \def\ermL{{\textnormal{L}}}
% \def\ermM{{\textnormal{M}}}
% \def\ermN{{\textnormal{N}}}
% \def\ermO{{\textnormal{O}}}
% \def\ermP{{\textnormal{P}}}
% \def\ermQ{{\textnormal{Q}}}
% \def\ermR{{\textnormal{R}}}
% \def\ermS{{\textnormal{S}}}
% \def\ermT{{\textnormal{T}}}
% \def\ermU{{\textnormal{U}}}
% \def\ermV{{\textnormal{V}}}
% \def\ermW{{\textnormal{W}}}
% \def\ermX{{\textnormal{X}}}
% \def\ermY{{\textnormal{Y}}}
% \def\ermZ{{\textnormal{Z}}}

% % Vectors
% \def\vzero{{\bm{0}}}
% \def\vone{{\bm{1}}}
% \def\vmu{{\bm{\mu}}}
% \def\vtheta{{\bm{\theta}}}
% \def\va{{\bm{a}}}
% \def\vb{{\bm{b}}}
% \def\vc{{\bm{c}}}
% \def\vd{{\bm{d}}}
% \def\ve{{\bm{e}}}
% \def\vf{{\bm{f}}}
% \def\vg{{\bm{g}}}
% \def\vh{{\bm{h}}}
% \def\vi{{\bm{i}}}
% \def\vj{{\bm{j}}}
% \def\vk{{\bm{k}}}
% \def\vl{{\bm{l}}}
% \def\vm{{\bm{m}}}
% \def\vn{{\bm{n}}}
% \def\vo{{\bm{o}}}
% \def\vp{{\bm{p}}}
% \def\vq{{\bm{q}}}
% \def\vr{{\bm{r}}}
% \def\vs{{\bm{s}}}
% \def\vt{{\bm{t}}}
% \def\vu{{\bm{u}}}
% \def\vv{{\bm{v}}}
% \def\vw{{\bm{w}}}
% \def\vx{{\bm{x}}}
% \def\vy{{\bm{y}}}
% \def\vz{{\bm{z}}}

% % Elements of vectors
% \def\evalpha{{\alpha}}
% \def\evbeta{{\beta}}
% \def\evepsilon{{\epsilon}}
% \def\evlambda{{\lambda}}
% \def\evomega{{\omega}}
% \def\evmu{{\mu}}
% \def\evpsi{{\psi}}
% \def\evsigma{{\sigma}}
% \def\evtheta{{\theta}}
% \def\eva{{a}}
% \def\evb{{b}}
% \def\evc{{c}}
% \def\evd{{d}}
% \def\eve{{e}}
% \def\evf{{f}}
% \def\evg{{g}}
% \def\evh{{h}}
% \def\evi{{i}}
% \def\evj{{j}}
% \def\evk{{k}}
% \def\evl{{l}}
% \def\evm{{m}}
% \def\evn{{n}}
% \def\evo{{o}}
% \def\evp{{p}}
% \def\evq{{q}}
% \def\evr{{r}}
% \def\evs{{s}}
% \def\evt{{t}}
% \def\evu{{u}}
% \def\evv{{v}}
% \def\evw{{w}}
% \def\evx{{x}}
% \def\evy{{y}}
% \def\evz{{z}}

% % Matrix
% \def\mA{{\bm{A}}}
% \def\mB{{\bm{B}}}
% \def\mC{{\bm{C}}}
% \def\mD{{\bm{D}}}
% \def\mE{{\bm{E}}}
% \def\mF{{\bm{F}}}
% \def\mG{{\bm{G}}}
% \def\mH{{\bm{H}}}
% \def\mI{{\bm{I}}}
% \def\mJ{{\bm{J}}}
% \def\mK{{\bm{K}}}
% \def\mL{{\bm{L}}}
% \def\mM{{\bm{M}}}
% \def\mN{{\bm{N}}}
% \def\mO{{\bm{O}}}
% \def\mP{{\bm{P}}}
% \def\mQ{{\bm{Q}}}
% \def\mR{{\bm{R}}}
% \def\mS{{\bm{S}}}
% \def\mT{{\bm{T}}}
% \def\mU{{\bm{U}}}
% \def\mV{{\bm{V}}}
% \def\mW{{\bm{W}}}
% \def\mX{{\bm{X}}}
% \def\mY{{\bm{Y}}}
% \def\mZ{{\bm{Z}}}
% \def\mBeta{{\bm{\beta}}}
% \def\mPhi{{\bm{\Phi}}}
% \def\mLambda{{\bm{\Lambda}}}
% \def\mSigma{{\bm{\Sigma}}}

% % Tensor
% \DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
% \SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
% \newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
% \def\tA{{\tens{A}}}
% \def\tB{{\tens{B}}}
% \def\tC{{\tens{C}}}
% \def\tD{{\tens{D}}}
% \def\tE{{\tens{E}}}
% \def\tF{{\tens{F}}}
% \def\tG{{\tens{G}}}
% \def\tH{{\tens{H}}}
% \def\tI{{\tens{I}}}
% \def\tJ{{\tens{J}}}
% \def\tK{{\tens{K}}}
% \def\tL{{\tens{L}}}
% \def\tM{{\tens{M}}}
% \def\tN{{\tens{N}}}
% \def\tO{{\tens{O}}}
% \def\tP{{\tens{P}}}
% \def\tQ{{\tens{Q}}}
% \def\tR{{\tens{R}}}
% \def\tS{{\tens{S}}}
% \def\tT{{\tens{T}}}
% \def\tU{{\tens{U}}}
% \def\tV{{\tens{V}}}
% \def\tW{{\tens{W}}}
% \def\tX{{\tens{X}}}
% \def\tY{{\tens{Y}}}
% \def\tZ{{\tens{Z}}}


% % Graph
% \def\gA{{\mathcal{A}}}
% \def\gB{{\mathcal{B}}}
% \def\gC{{\mathcal{C}}}
% \def\gD{{\mathcal{D}}}
% \def\gE{{\mathcal{E}}}
% \def\gF{{\mathcal{F}}}
% \def\gG{{\mathcal{G}}}
% \def\gH{{\mathcal{H}}}
% \def\gI{{\mathcal{I}}}
% \def\gJ{{\mathcal{J}}}
% \def\gK{{\mathcal{K}}}
% \def\gL{{\mathcal{L}}}
% \def\gM{{\mathcal{M}}}
% \def\gN{{\mathcal{N}}}
% \def\gO{{\mathcal{O}}}
% \def\gP{{\mathcal{P}}}
% \def\gQ{{\mathcal{Q}}}
% \def\gR{{\mathcal{R}}}
% \def\gS{{\mathcal{S}}}
% \def\gT{{\mathcal{T}}}
% \def\gU{{\mathcal{U}}}
% \def\gV{{\mathcal{V}}}
% \def\gW{{\mathcal{W}}}
% \def\gX{{\mathcal{X}}}
% \def\gY{{\mathcal{Y}}}
% \def\gZ{{\mathcal{Z}}}

% % Sets
% \def\sA{{\mathbb{A}}}
% \def\sB{{\mathbb{B}}}
% \def\sC{{\mathbb{C}}}
% \def\sD{{\mathbb{D}}}
% % Don't use a set called E, because this would be the same as our symbol
% % for expectation.
% \def\sF{{\mathbb{F}}}
% \def\sG{{\mathbb{G}}}
% \def\sH{{\mathbb{H}}}
% \def\sI{{\mathbb{I}}}
% \def\sJ{{\mathbb{J}}}
% \def\sK{{\mathbb{K}}}
% \def\sL{{\mathbb{L}}}
% \def\sM{{\mathbb{M}}}
% \def\sN{{\mathbb{N}}}
% \def\sO{{\mathbb{O}}}
% \def\sP{{\mathbb{P}}}
% \def\sQ{{\mathbb{Q}}}
% \def\sR{{\mathbb{R}}}
% \def\sS{{\mathbb{S}}}
% \def\sT{{\mathbb{T}}}
% \def\sU{{\mathbb{U}}}
% \def\sV{{\mathbb{V}}}
% \def\sW{{\mathbb{W}}}
% \def\sX{{\mathbb{X}}}
% \def\sY{{\mathbb{Y}}}
% \def\sZ{{\mathbb{Z}}}

% % Entries of a matrix
% \def\emLambda{{\Lambda}}
% \def\emA{{A}}
% \def\emB{{B}}
% \def\emC{{C}}
% \def\emD{{D}}
% \def\emE{{E}}
% \def\emF{{F}}
% \def\emG{{G}}
% \def\emH{{H}}
% \def\emI{{I}}
% \def\emJ{{J}}
% \def\emK{{K}}
% \def\emL{{L}}
% \def\emM{{M}}
% \def\emN{{N}}
% \def\emO{{O}}
% \def\emP{{P}}
% \def\emQ{{Q}}
% \def\emR{{R}}
% \def\emS{{S}}
% \def\emT{{T}}
% \def\emU{{U}}
% \def\emV{{V}}
% \def\emW{{W}}
% \def\emX{{X}}
% \def\emY{{Y}}
% \def\emZ{{Z}}
% \def\emSigma{{\Sigma}}

% % entries of a tensor
% % Same font as tensor, without \bm wrapper
% \newcommand{\etens}[1]{\mathsfit{#1}}
% \def\etLambda{{\etens{\Lambda}}}
% \def\etA{{\etens{A}}}
% \def\etB{{\etens{B}}}
% \def\etC{{\etens{C}}}
% \def\etD{{\etens{D}}}
% \def\etE{{\etens{E}}}
% \def\etF{{\etens{F}}}
% \def\etG{{\etens{G}}}
% \def\etH{{\etens{H}}}
% \def\etI{{\etens{I}}}
% \def\etJ{{\etens{J}}}
% \def\etK{{\etens{K}}}
% \def\etL{{\etens{L}}}
% \def\etM{{\etens{M}}}
% \def\etN{{\etens{N}}}
% \def\etO{{\etens{O}}}
% \def\etP{{\etens{P}}}
% \def\etQ{{\etens{Q}}}
% \def\etR{{\etens{R}}}
% \def\etS{{\etens{S}}}
% \def\etT{{\etens{T}}}
% \def\etU{{\etens{U}}}
% \def\etV{{\etens{V}}}
% \def\etW{{\etens{W}}}
% \def\etX{{\etens{X}}}
% \def\etY{{\etens{Y}}}
% \def\etZ{{\etens{Z}}}

% % The true underlying data generating distribution
% \newcommand{\pdata}{p_{\rm{data}}}
% % The empirical distribution defined by the training set
% \newcommand{\ptrain}{\hat{p}_{\rm{data}}}
% \newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% % The model distribution
% \newcommand{\pmodel}{p_{\rm{model}}}
% \newcommand{\Pmodel}{P_{\rm{model}}}
% \newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% % Stochastic autoencoder distributions
% \newcommand{\pencode}{p_{\rm{encoder}}}
% \newcommand{\pdecode}{p_{\rm{decoder}}}
% \newcommand{\precons}{p_{\rm{reconstruct}}}

% \newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
% \newcommand{\Ls}{\mathcal{L}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\emp}{\tilde{p}}
% \newcommand{\lr}{\alpha}
% \newcommand{\reg}{\lambda}
% \newcommand{\rect}{\mathrm{rectifier}}
% \newcommand{\softmax}{\mathrm{softmax}}
% \newcommand{\sigmoid}{\sigma}
% \newcommand{\softplus}{\zeta}
% \newcommand{\KL}{D_{\mathrm{KL}}}
% \newcommand{\Var}{\mathrm{Var}}
% \newcommand{\standarderror}{\mathrm{SE}}
% \newcommand{\Cov}{\mathrm{Cov}}
% % Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% % But then they seem to use $L^2$ for vectors throughout the site, and so does
% % wikipedia.
% \newcommand{\normlzero}{L^0}
% \newcommand{\normlone}{L^1}
% \newcommand{\normltwo}{L^2}
% \newcommand{\normlp}{L^p}
% \newcommand{\normmax}{L^\infty}

% \newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \DeclareMathOperator{\sign}{sign}
% \DeclareMathOperator{\Tr}{Tr}
% \let\ab\allowbreak

